MCIF: Multimodal Crosslingual Instruction-Following Benchmark from Scientific Talks

Recent advances in large language models have laid the foundation for multimodal LLMs (MLLMs), which unify text, speech, and vision within a single framework. As these models are rapidly evolving toward general-purpose instruction following across diverse and complex tasks, a key frontier is evaluating their crosslingual and multimodal capabilities over both short- and long-form inputs. However, existing benchmarks fall short in evaluating these dimensions jointly: they are often limited to English, mostly focus on a single modality at a time, rely on short-form inputs, or lack human annotations--hindering comprehensive assessment of model performance across languages, modalities, and task complexity. To address these gaps, we introduce MCIF (Multimodal Crosslingual Instruction Following), the first crosslingual human-annotated benchmark based on scientific talks on NLP and beyond. MCIF evaluates instruction following in crosslingual, multimodal settings over different input lengths and spans four macro-tasks: recognition, translation, question answering, and summarization. It covers three core modalities (speech, vision, and text) and four diverse languages (English, German, Italian, and Chinese), fully aligned across all dimensions. This parallel design enables a systematic evaluation of MLLMs' abilities to interpret instructions across languages and effectively integrate multimodal contextual information. Our benchmarking and analysis of 23 models highlight universal challenges across modalities and tasks, indicating substantial room for improvement in future MLLMs development. MCIF is released under CC-BY 4.0 license to promote open research.

==> results.tex <==
% In this section, we report the results on \DATASETNAME{} from several perspectives. First, in \cref{subsec:fix_mix}, we analyze the overall performance achieved by all the \NMODELS{} models. Subsequently, in \cref{subsec:modalities}, we focus on MLLMs and investigate the impact of different modalities on the model's abilities to perform each task. Lastly, in \cref{subsec:questions}, we isolate the question answering task and break down the results of the best-performing model for each category (LLM, SpeechLLM, VideoLLM, and MLLM), considering the type of question and the input modality required to answer the question.
This section reports results on \DATASETNAME{} from several perspectives: \cref{subsec:fix_mix} analyzes overall performance across all \NMODELS{} models and macro-tasks, \cref{subsec:modalities} focuses on MLLMs to study how different modalities impact task performance, and \cref{subsec:questions} studies how the best model in each category (LLM, SpeechLLM, VideoLLM, MLLM) performs on question answering across question types.

\subsection{Overall Results}
\label{subsec:fix_mix}

% \cref{tab:main_fix} and \cref{tab:main_mix} report the model results on \MCIFFIX{} and \MCIFMIX{}, respectively, for each model, context (long or short), and task divided by macro-area. We also report the non-normalized BERTScore results for question answering and summarization tasks in \cref{app:non-norm}.

\cref{tab:overall} reports the model results on \MCIFFIX{} and \MCIFMIX{} for each context (long or short), and macro-task. Extended results per language are reported in \cref{app:mcif_extended}. 
% We also report the non-normalized BERTScore results for question answering and summarization tasks in \cref{app:non-norm}.


%===================
\begin{table}[h]
\centering
    \resizebox{\linewidth}{!}{%
    \setlength{\tabcolsep}{3.5pt} 
\begin{tabular}{c|c|c|cccc|cccc}
\toprule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{Context}}} & \multirow{3}{*}{\shortstack{\textbf{Input}\\\textbf{Modality}}} & \multirow{3}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{\MCIFFIX{}}} & \multicolumn{4}{c}{\textbf{\MCIFMIX{}}} \\
 &  &  & \REClabel{} & \TRANSlabel{} & \QAlabel{} & \SUMlabel{} & \REClabel{} & \TRANSlabel{} & \QAlabel{} & \SUMlabel{} \\
 &  &  & WER↓ & COMET↑ & BERTS.↑ & BERTS.↑ & WER↓ & COMET↑ & BERTS.↑ & BERTS.↑ \\
\midrule
\multirow{15}{*}{\rotatebox[origin=c]{90}{\scalebox{1.5}\shortin{}}} & \multirow{5}{*}{{\scalebox{2}\speechmod{}}} & \hyperlink{desta2}{DeSTA2} & \heatRECval{54.0} & \heatTRANSval{75.3} & \heatQAval{17.2} & \multirow{5}{*}{\texttimes} & \heatRECval{83.0} & \heatTRANSval{75.2} & \heatQAval{18.6} & \multirow{5}{*}{\texttimes} \\
 &  & \hyperlink{granite}{GraniteSpeech} & \heatRECval{9.4} & \heatTRANSval{52.1} & \heatQAval{0.5} &  & \heatRECval{9.5} & \heatTRANSval{46.6} & \heatQAval{0.4} & \\
 &  & \hyperlink{phi4m}{Phi4-Multimodal} & \textbf{\underline{\heatRECval{6.8}}} & \textbf{\heatTRANSval{80.2}} & \heatQAval{37.1} &  & \textbf{\heatRECval{6.7}} & \textbf{\heatTRANSval{80.1}} & \heatQAval{37.4} &  \\
  &  & \hyperlink{qwen2a}{Qwen2-Audio} & \heatRECval{31.7} & \heatTRANSval{74.9} & \heatQAval{32.6} &  & \heatRECval{31.9} & \heatTRANSval{74.6} & \heatQAval{32.8} & \\
 &  & \hyperlink{ultravox}{UltraVox v0.5} & \heatRECval{127.7} & \heatTRANSval{43.3} & \heatQAval{19.6} &  & \heatRECval{172.6} & \heatTRANSval{43.2} & \heatQAval{19.1} & \\
 \cmidrule{2-11}
 & \multirow{5}{*}{{\scalebox{2}\videomod{}}} & \hyperlink{internvl3}{InternVL3} & \multicolumn{2}{c}{\multirow{5}{*}{\texttimes}} & \heatQAval{31.7} & \multirow{5}{*}{\texttimes} & \multicolumn{2}{c}{\multirow{5}{*}{\texttimes}} & \heatQAval{31.3} & \multirow{5}{*}{\texttimes} \\
&  & \hyperlink{llavanv}{LLaVA-NeXT} & & & \heatQAval{13.7} & & & & \heatQAval{12.1} & \\
 &  & \hyperlink{qwen2.5vl}{Qwen2.5-VL} & & & \heatQAval{39.1} & & & & \heatQAval{37.8} & \\
 &  & \hyperlink{videollama3}{VideoLLaMA3} & & & \heatQAval{24.1} & & & & \heatQAval{23.8} & \\
 &  & \hyperlink{videoxl2}{Video-XL2} & & & \heatQAval{13.6} & & & & \heatQAval{13.6} & \\
 \cmidrule{2-11}
& \multirow{5}{*}{{\scalebox{1.75}\speechmod{}\scalebox{1.75}\videomod{}}} & \hyperlink{gemma3n}{Gemma 3n} & \heatRECval{35.1} & \heatTRANSval{73.0} & \heatQAval{26.2} & \multirow{6}{*}{\texttimes} & \heatRECval{58.9} & \heatTRANSval{71.5} & \heatQAval{25.1} & \multirow{6}{*}{\texttimes} \\
 &  & \hyperlink{ming}{Ming-Lite-Omni} & \heatRECval{117.5} & \heatTRANSval{53.0} & \heatQAval{15.8} & & \heatRECval{128.2} & \heatTRANSval{53.3} & \heatQAval{13.3} & \\
 &  & \hyperlink{minicpm}{MiniCPM-o-2} & \heatRECval{144.8} & \heatTRANSval{39.7} & \heatQAval{21.4} & & \heatRECval{207.1} & \heatTRANSval{38.8} & \heatQAval{23.1} & \\
 &  & \hyperlink{ola}{Ola} & \heatRECval{104.1} & \heatTRANSval{76.6} & \heatQAval{37.3} &  & \heatRECval{98.8} & \heatTRANSval{76.3} & \heatQAval{37.0} &  \\
 &  & \hyperlink{qwen2.5omni}{Qwen2.5-Omni} & \heatRECval{43.5} & \heatTRANSval{77.3} & \heatQAval{34.3} &  & \heatRECval{48.0} & \heatTRANSval{76.5} & \heatQAval{35.1} & \\
 & & \textit{Gemini 2.5 Flash} & \heatRECval{14.9} & \heatTRANSval{67.0} & \textbf{\heatQAval{40.6}} & \multirow{5}{*}{\texttimes} & \heatRECval{12.8} & \heatTRANSval{69.2} & \textbf{\heatQAval{39.5}} & \multirow{5}{*}{\texttimes} \\
\midrule
\midrule
\multirow{19}{*}{\rotatebox[origin=c]{90}{\scalebox{1.5}\longin{}}} & \multirow{7}{*}{{\scalebox{2}\textmod{}}} & \hyperlink{aya}{Aya Expanse} & \multirow{7}{*}{\texttimes}  & \heatTRANSval{68.7} & \heatQAval{26.7} & \heatSUMval{17.1} & \multirow{7}{*}{\texttimes} & \heatTRANSval{68.7} & \heatQAval{23.1} & \heatSUMval{16.3} \\
 &  & \hyperlink{gemma3}{Gemma 3} &  & \heatTRANSval{85.5} & \heatQAval{22.9} & \heatSUMval{5.4} &  & \heatTRANSval{83.4} & \heatQAval{21.8} & \heatSUMval{5.2} \\
 &  & \hyperlink{gptoss}{GPT-oss} &  & \heatTRANSval{75.0} & \heatQAval{24.6} & \heatSUMval{10.5} &  & \heatTRANSval{70.1} & \heatQAval{20.9} & \heatSUMval{9.0} \\
&  & \hyperlink{llama3}{Llama 3.1} &  & \heatTRANSval{81.4} & \heatQAval{30.3} & \textbf{\underline{\heatSUMval{17.9}}} &  & \heatTRANSval{79.5} & \heatQAval{31.0} & \textbf{\underline{\heatSUMval{17.2}}} \\
 &  & \hyperlink{phi4}{Phi4} &  & \heatTRANSval{84.5} & \heatQAval{30.8} & \heatSUMval{7.4} &  & \textbf{\underline{\heatTRANSval{84.7}}} & \heatQAval{29.6} & \heatSUMval{8.5} \\
 &  & \hyperlink{qwen3}{Qwen3} &  & \heatTRANSval{84.8} & \heatQAval{37.9} & \heatSUMval{14.0} &  & \heatTRANSval{84.5} & \heatQAval{35.6} & \heatSUMval{14.0} \\
 &  & \hyperlink{tower}{Tower+} &  & \textbf{\underline{\heatTRANSval{85.6}}} & \heatQAval{29.5} & \heatSUMval{13.3} &  & \heatTRANSval{83.7} & \heatQAval{23.4} & \heatSUMval{11.2} \\
 \cmidrule{2-11}
 & \multirow{5}{*}{{\scalebox{2}\speechmod{}}} & \hyperlink{desta2}{DeSTA2} & \heatRECval{112.9} & \heatTRANSval{41.3} & \heatQAval{12.5} & \heatSUMval{1.0} & \heatRECval{132.5} & \heatTRANSval{40.8} & \heatQAval{12.6} & \heatSUMval{1.4} \\
 &  & \hyperlink{granite}{GraniteSpeech} & \heatRECval{99.9} & \heatTRANSval{36.0} & \heatQAval{-23.7} & \heatSUMval{0.8} & \heatRECval{80.4} & \heatTRANSval{34.6} & \heatQAval{-22.8} & \heatSUMval{-12.1} \\
 &  & \hyperlink{phi4m}{Phi4-Multimodal} & \heatRECval{39.2} & \heatTRANSval{59.7} & \heatQAval{37.6} & \heatSUMval{4.9} & \heatRECval{29.8} & \heatTRANSval{59.5} & \heatQAval{37.3} & \heatSUMval{13.2} \\
  &  & \hyperlink{qwen2a}{Qwen2-Audio} & \heatRECval{92.9} & \heatTRANSval{41.0} & \heatQAval{28.8} & \heatSUMval{5.1} & \heatRECval{93.1} & \heatTRANSval{41.1} & \heatQAval{28.9} & \heatSUMval{4.7} \\
 &  & \hyperlink{ultravox}{UltraVox v0.5} & \heatRECval{89.1} & \heatTRANSval{38.0} & \heatQAval{12.7} & \heatSUMval{-3.5} & \heatRECval{92.5} & \heatTRANSval{38.0} & \heatQAval{12.5} & \heatSUMval{-3.6} \\
 \cmidrule{2-11}
 & \multirow{5}{*}{{\scalebox{2}\videomod{}}} & \hyperlink{internvl3}{InternVL3} & \multicolumn{2}{c}{\multirow{5}{*}{\texttimes}} & \heatQAval{27.6} & \heatSUMval{15.3} & \multicolumn{2}{c}{\multirow{5}{*}{\texttimes}} & \heatQAval{27.9} & \heatSUMval{15.0} \\
&  & \hyperlink{llavanv}{LLaVA-NeXT} & \multicolumn{2}{c}{} & \heatQAval{7.2} & \heatSUMval{-7.8} & & & \heatQAval{5.2} & \heatSUMval{-7.4} \\
 &  & \hyperlink{qwen2.5vl}{Qwen2.5-VL} & \multicolumn{2}{c}{} & \heatQAval{33.7} & \heatSUMval{17.6} & & & \heatQAval{34.9} & \heatSUMval{14.7} \\
 &  & \hyperlink{videollama3}{VideoLLaMA3} & \multicolumn{2}{c}{} & \heatQAval{26.8} & \heatSUMval{-22.2} & & & \heatQAval{26.5} & \heatSUMval{-34.7} \\
 &  & \hyperlink{videoxl2}{Video-XL2} & \multicolumn{2}{c}{} & \heatQAval{17.2} & \heatSUMval{2.3} & & & \heatQAval{17.4} & \heatSUMval{2.9} \\
 \cmidrule{2-11}
 & \multirow{3}{*}{{\scalebox{1.75}\speechmod{}\scalebox{1.75}\videomod{}}} & \hyperlink{minicpm}{MiniCPM-o-2} & \heatRECval{98.7} & \heatTRANSval{39.1} & \heatQAval{21.5} & \heatSUMval{-40.7} & \heatRECval{98.2} & \heatTRANSval{39.1} & \heatQAval{22.9} & \heatSUMval{-40.4} \\
 &  & \hyperlink{ola}{Ola} & \heatRECval{14.0} & \heatTRANSval{63.2} & \heatQAval{36.2} & \heatSUMval{8.8} & \textbf{\underline{\heatRECval{6.6}}} & \heatTRANSval{58.7} & \heatQAval{36.2} & \heatSUMval{10.0} \\
 &  & \hyperlink{qwen2.5omni}{Qwen2.5-Omni} & \heatRECval{98.5} & \heatTRANSval{47.5} & \heatQAval{32.5} & \heatSUMval{6.1} & \heatRECval{94.9} & \heatTRANSval{40.2} & \heatQAval{34.8} & \heatSUMval{6.0} \\
 &  & \textit{Gemini 2.5 Flash} & \textbf{\heatRECval{11.9}} & \heatTRANSval{76.4} & \textbf{\underline{\heatQAval{46.1}}} & \heatSUMval{15.4} & \heatRECval{7.9} & \heatTRANSval{79.9} & \textbf{\underline{\heatQAval{45.9}}} & \heatSUMval{13.8} \\
 \bottomrule
\end{tabular}}
\caption{Overall results, averaged across languages, on \MCIFFIX{} and \MCIFMIX{}, divided into the four macro-tasks: recognition (\textbf{REC}), translation (\textbf{TRANS}), question answering (\textbf{QA}), and summarization (\textbf{SUM}). Best result by context is marked in \textbf{bold}, and best overall result is \underline{underlined}. \texttimes{} marks unfeasible tasks, i.e., summarization with short-form, or out of models' scope for a given modality: recognition for LLMs and VideoLLMs (requires speech), and translation for VideoLLMs (requires speech or text). Gemma 3n and Ming-Lite-Omni are removed from \longin{} as they are not able to process long-form inputs.}
\label{tab:overall}
\end{table}

%===================SUBMISSION TABLE
% \begin{table}[h]
% \centering
%     \resizebox{\linewidth}{!}{%
%     \setlength{\tabcolsep}{3.5pt} 
% \begin{tabular}{c|c|c|cccc|cccc}
% \toprule
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{Context}}} & \multirow{3}{*}{\shortstack{\textbf{Input}\\\textbf{Modality}}} & \multirow{3}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{\MCIFFIX{}}} & \multicolumn{4}{c}{\textbf{\MCIFMIX{}}} \\
%  &  &  & \REClabel{} & \TRANSlabel{} & \QAlabel{} & \SUMlabel{} & \REClabel{} & \TRANSlabel{} & \QAlabel{} & \SUMlabel{} \\
%  &  &  & WER↓ & COMET↑ & BERTS.↑ & BERTS.↑ & WER↓ & COMET↑ & BERTS.↑ & BERTS.↑ \\
% \midrule
% \multirow{15}{*}{\rotatebox[origin=c]{90}{\scalebox{1.5}\shortin{}}} & \multirow{5}{*}{{\scalebox{2}\speechmod{}}} & \hyperlink{desta2}{DeSTA2} & \heatRECval{54.0} & \heatTRANSval{75.3} & \heatQAval{17.2} & \multirow{5}{*}{\texttimes} & \heatRECval{83.0} & \heatTRANSval{75.2} & \heatQAval{18.6} & \multirow{5}{*}{\texttimes} \\
%  &  & \hyperlink{granite}{GraniteSpeech} & \heatRECval{9.4} & \heatTRANSval{52.1} & \heatQAval{0.5} &  & \heatRECval{9.5} & \heatTRANSval{46.6} & \heatQAval{0.4} & \\
%  &  & \hyperlink{phi4m}{Phi4-Multimodal} & \textbf{\underline{\heatRECval{6.8}}} & \textbf{\heatTRANSval{80.2}} & \heatQAval{37.1} &  & \textbf{\heatRECval{6.7}} & \textbf{\heatTRANSval{80.1}} & \heatQAval{37.4} &  \\
%   &  & \hyperlink{qwen2a}{Qwen2-Audio} & \heatRECval{31.7} & \heatTRANSval{74.9} & \heatQAval{32.6} &  & \heatRECval{31.9} & \heatTRANSval{74.6} & \heatQAval{32.8} & \\
%  &  & \hyperlink{ultravox}{UltraVox v0.5} & \heatRECval{127.7} & \heatTRANSval{43.3} & \heatQAval{19.6} &  & \heatRECval{172.6} & \heatTRANSval{43.2} & \heatQAval{19.1} & \\
%  \cmidrule{2-11}
%  & \multirow{5}{*}{{\scalebox{2}\videomod{}}} & \hyperlink{internvl3}{InternVL3} & \multicolumn{2}{c}{\multirow{5}{*}{\texttimes}} & \heatQAval{31.7} & \multirow{5}{*}{\texttimes} & \multicolumn{2}{c}{\multirow{5}{*}{\texttimes}} & \heatQAval{31.3} & \multirow{5}{*}{\texttimes} \\
% &  & \hyperlink{llavanv}{LLaVA-NeXT} & & & \heatQAval{13.7} & & & & \heatQAval{12.1} & \\
%  &  & \hyperlink{qwen2.5vl}{Qwen2.5-VL} & & & \heatQAval{39.1} & & & & \heatQAval{37.8} & \\
%  &  & \hyperlink{videollama3}{VideoLLaMA3} & & & \heatQAval{24.1} & & & & \heatQAval{23.8} & \\
%  &  & \hyperlink{videoxl2}{Video-XL2} & & & \heatQAval{13.6} & & & & \heatQAval{13.6} & \\
%  \cmidrule{2-11}
% & \multirow{5}{*}{{\scalebox{1.75}\speechmod{}\scalebox{1.75}\videomod{}}} & \hyperlink{gemma3n}{Gemma 3n} & \heatRECval{35.1} & \heatTRANSval{73.0} & \heatQAval{26.2} & \multirow{6}{*}{\texttimes} & \heatRECval{58.9} & \heatTRANSval{71.5} & \heatQAval{25.1} & \multirow{6}{*}{\texttimes} \\
%  &  & \hyperlink{ming}{Ming-Lite-Omni} & \heatRECval{117.5} & \heatTRANSval{53.0} & \heatQAval{15.8} & & \heatRECval{128.2} & \heatTRANSval{53.3} & \heatQAval{13.3} & \\
%  &  & \hyperlink{minicpm}{MiniCPM-o-2} & \heatRECval{144.8} & \heatTRANSval{39.7} & \heatQAval{21.4} & & \heatRECval{207.1} & \heatTRANSval{38.8} & \heatQAval{23.1} & \\
%  &  & \hyperlink{ola}{Ola} & \heatRECval{104.1} & \heatTRANSval{76.6} & \heatQAval{37.3} &  & \heatRECval{98.8} & \heatTRANSval{76.3} & \heatQAval{37.0} &  \\
%  &  & \hyperlink{qwen2.5omni}{Qwen2.5-Omni} & \heatRECval{43.5} & \heatTRANSval{77.3} & \heatQAval{34.3} &  & \heatRECval{48.0} & \heatTRANSval{76.5} & \heatQAval{35.1} & \\
%  & & \textit{Gemini 2.5 Flash} & \heatRECval{14.9} & \heatTRANSval{67.0} & \textbf{\heatQAval{40.6}} & \multirow{5}{*}{\texttimes} & \heatRECval{12.8} & \heatTRANSval{69.2} & \textbf{\heatQAval{39.5}} & \multirow{5}{*}{\texttimes} \\
% \midrule
% \midrule
% \multirow{19}{*}{\rotatebox[origin=c]{90}{\scalebox{1.5}\longin{}}} & \multirow{7}{*}{{\scalebox{2}\textmod{}}} & \hyperlink{aya}{Aya Expanse} & \multirow{7}{*}{\texttimes}  & \heatTRANSval{68.7} & \heatQAval{26.7} & \heatSUMval{17.0} & \multirow{7}{*}{\texttimes} & \heatTRANSval{68.7} & \heatQAval{23.1} & \heatSUMval{16.3} \\
%  &  & \hyperlink{gemma3}{Gemma 3} &  & \heatTRANSval{85.5} & \heatQAval{22.9} & \heatSUMval{5.6} &  & \heatTRANSval{83.4} & \heatQAval{21.8} & \heatSUMval{5.2} \\
%  &  & \hyperlink{gptoss}{GPT-oss} &  & \heatTRANSval{75.0} & \heatQAval{24.6} & \heatSUMval{10.5} &  & \heatTRANSval{70.1} & \heatQAval{20.9} & \heatSUMval{9.2} \\
% &  & \hyperlink{llama3}{Llama 3.1} &  & \heatTRANSval{81.4} & \heatQAval{30.3} & \textbf{\underline{\heatSUMval{18.1}}} &  & \heatTRANSval{79.5} & \heatQAval{31.0} & \textbf{\underline{\heatSUMval{17.3}}} \\
%  &  & \hyperlink{phi4}{Phi4} &  & \heatTRANSval{84.5} & \heatQAval{30.8} & \heatSUMval{7.3} &  & \textbf{\underline{\heatTRANSval{84.7}}} & \heatQAval{29.6} & \heatSUMval{8.4} \\
%  &  & \hyperlink{qwen3}{Qwen3} &  & \heatTRANSval{84.8} & \heatQAval{37.9} & \heatSUMval{14.1} &  & \heatTRANSval{84.5} & \heatQAval{35.6} & \heatSUMval{14.0} \\
%  &  & \hyperlink{tower}{Tower+} &  & \textbf{\underline{\heatTRANSval{85.6}}} & \heatQAval{29.5} & \heatSUMval{13.4} &  & \heatTRANSval{83.7} & \heatQAval{23.4} & \heatSUMval{11.2} \\
%  \cmidrule{2-11}
%  & \multirow{5}{*}{{\scalebox{2}\speechmod{}}} & \hyperlink{desta2}{DeSTA2} & \heatRECval{112.9} & \heatTRANSval{41.3} & \heatQAval{12.5} & \heatSUMval{0.8} & \heatRECval{132.5} & \heatTRANSval{40.8} & \heatQAval{12.6} & \heatSUMval{1.3} \\
%  &  & \hyperlink{granite}{GraniteSpeech} & \heatRECval{99.9} & \heatTRANSval{36.0} & \heatQAval{-23.7} & \heatSUMval{0.4} & \heatRECval{80.4} & \heatTRANSval{34.6} & \heatQAval{-22.8} & \heatSUMval{-12.0} \\
%  &  & \hyperlink{phi4m}{Phi4-Multimodal} & \heatRECval{39.2} & \heatTRANSval{59.7} & \heatQAval{37.6} & \heatSUMval{4.5} & \heatRECval{29.8} & \heatTRANSval{59.5} & \heatQAval{37.3} & \heatSUMval{13.2} \\
%   &  & \hyperlink{qwen2a}{Qwen2-Audio} & \heatRECval{92.9} & \heatTRANSval{41.0} & \heatQAval{28.8} & \heatSUMval{4.6} & \heatRECval{93.1} & \heatTRANSval{41.1} & \heatQAval{28.9} & \heatSUMval{4.6} \\
%  &  & \hyperlink{ultravox}{UltraVox v0.5} & \heatRECval{89.1} & \heatTRANSval{38.0} & \heatQAval{12.7} & \heatSUMval{-3.8} & \heatRECval{92.5} & \heatTRANSval{38.0} & \heatQAval{12.5} & \heatSUMval{-3.9} \\
%  \cmidrule{2-11}
%  & \multirow{5}{*}{{\scalebox{2}\videomod{}}} & \hyperlink{internvl3}{InternVL3} & \multicolumn{2}{c}{\multirow{5}{*}{\texttimes}} & \heatQAval{27.6} & \heatSUMval{15.4} & \multicolumn{2}{c}{\multirow{5}{*}{\texttimes}} & \heatQAval{27.9} & \heatSUMval{14.8} \\
% &  & \hyperlink{llavanv}{LLaVA-NeXT} & \multicolumn{2}{c}{} & \heatQAval{7.2} & \heatSUMval{-7.9} & & & \heatQAval{5.2} & \heatSUMval{-7.4} \\
%  &  & \hyperlink{qwen2.5vl}{Qwen2.5-VL} & \multicolumn{2}{c}{} & \heatQAval{33.7} & \heatSUMval{17.3} & & & \heatQAval{34.9} & \heatSUMval{14.6} \\
%  &  & \hyperlink{videollama3}{VideoLLaMA3} & \multicolumn{2}{c}{} & \heatQAval{26.8} & \heatSUMval{-18.5} & & & \heatQAval{26.5} & \heatSUMval{-34.6} \\
%  &  & \hyperlink{videoxl2}{Video-XL2} & \multicolumn{2}{c}{} & \heatQAval{17.2} & \heatSUMval{2.1} & & & \heatQAval{17.4} & \heatSUMval{2.8} \\
%  \cmidrule{2-11}
%  & \multirow{3}{*}{{\scalebox{1.75}\speechmod{}\scalebox{1.75}\videomod{}}} & \hyperlink{minicpm}{MiniCPM-o-2} & \heatRECval{98.7} & \heatTRANSval{39.1} & \heatQAval{21.5} & \heatSUMval{-3.2} & \heatRECval{98.2} & \heatTRANSval{39.1} & \heatQAval{22.9} & \heatSUMval{-4.0} \\
%  &  & \hyperlink{ola}{Ola} & \heatRECval{14.0} & \heatTRANSval{63.2} & \heatQAval{36.2} & \heatSUMval{8.8} & \textbf{\underline{\heatRECval{6.6}}} & \heatTRANSval{58.7} & \heatQAval{36.2} & \heatSUMval{9.9} \\
%  &  & \hyperlink{qwen2.5omni}{Qwen2.5-Omni} & \heatRECval{98.5} & \heatTRANSval{47.5} & \heatQAval{32.5} & \heatSUMval{6.1} & \heatRECval{94.9} & \heatTRANSval{40.2} & \heatQAval{34.8} & \heatSUMval{6.0} \\
%  &  & \textit{Gemini 2.5 Flash} & \textbf{\heatRECval{11.9}} & \heatTRANSval{76.4} & \textbf{\underline{\heatQAval{46.1}}} & \heatSUMval{15.9} & \heatRECval{7.9} & \heatTRANSval{79.9} & \textbf{\underline{\heatQAval{45.9}}} & \heatSUMval{13.8} \\
%  \bottomrule
% \end{tabular}}
% \caption{Overall results, averaged across languages, on \MCIFFIX{} and \MCIFMIX{}, divided into the four macro-tasks: recognition (\textbf{REC}), translation (\textbf{TRANS}), question answering (\textbf{QA}), and summarization (\textbf{SUM}). Best result by context is marked in \textbf{bold}, and best overall result is \underline{underlined}. \texttimes{} marks unfeasible tasks, i.e., summarization with short-form, or out of models' scope for a given modality: recognition for LLMs and VideoLLMs (requires speech), and translation for VideoLLMs (requires speech or text). Gemma 3n and Ming-Lite-Omni are removed from \longin{} as they are not able to process long-form inputs.}
% \label{tab:overall}
% \end{table}


%================= UNCOLORED TABLE

% \begin{table}[h]
% \centering
%     \resizebox{\linewidth}{!}{%
%     \setlength{\tabcolsep}{3pt} 
% \begin{tabular}{c|c|c|cccc|cccc}
% \toprule
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{Context}}} & \multirow{3}{*}{\shortstack{\textbf{Input}\\\textbf{Modality}}} & \multirow{3}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{\MCIFFIX{}}} & \multicolumn{4}{c}{\textbf{\MCIFMIX{}}} \\
%  &  &  & \textbf{REC} & \textbf{TRANS} & \textbf{QA} & \textbf{SUM} & \textbf{REC} & \textbf{TRANS} & \textbf{QA} & \textbf{SUM} \\
%  &  &  & WER↓ & COMET↑ & BERTS.↑ & BERTS.↑ & WER↓ & COMET↑ & BERTS.↑ & BERTS.↑ \\
% \midrule
% \multirow{15}{*}{\rotatebox[origin=c]{90}{\scalebox{1.5}\shortin{}}} & \multirow{5}{*}{{\scalebox{2}\speechmod{}}} & \hyperlink{desta2}{DeSTA2} & 54.0 & 75.3 & 17.2 & \multirow{5}{*}{\texttimes} & 83.0 & 75.2 & 18.6 & \multirow{5}{*}{\texttimes} \\
%  &  & \hyperlink{granite}{GraniteSpeech} & 9.4 & 52.1 & 0.5 &  & 9.5 & 46.6 & 0.4 & \\
%  &  & \hyperlink{phi4m}{Phi4-Multimodal} & \textbf{\underline{6.8}} & \textbf{80.2} & 37.1 &  & \textbf{6.7} & \textbf{80.1} & 37.4 &  \\
%   &  & \hyperlink{qwen2a}{Qwen2-Audio} & 31.7 & 74.9 & 32.6 &  & 31.9 & 74.6 & 32.8 & \\
%  &  & \hyperlink{ultravox}{UltraVox v0.5} & 127.7 & 43.3 & 19.6 &  & 172.6 & 43.2 & 19.1 & \\
%  \cmidrule{2-11}
%  & \multirow{5}{*}{{\scalebox{2}\videomod{}}} & \hyperlink{internvl3}{InternVL3} & \multicolumn{2}{c}{\multirow{5}{*}{\texttimes}} & 31.7 & \multirow{5}{*}{\texttimes} & \multicolumn{2}{c}{\multirow{5}{*}{\texttimes}} & 31.3 & \multirow{5}{*}{\texttimes} \\
% &  & \hyperlink{llavanv}{LLaVA-NeXT} & & & 13.7 & & & & 12.1 & \\
%  &  & \hyperlink{qwen2.5vl}{Qwen2.5-VL} & & & \textbf{\underline{39.1}} & & & & \textbf{\underline{37.8}} & \\
%  &  & \hyperlink{videollama3}{VideoLLaMA3} & & & 24.1 & & & & 23.8 & \\
%  &  & \hyperlink{videoxl2}{Video-XL2} & & & 13.6 & & & & 13.6 & \\
%  \cmidrule{2-11}
% & \multirow{5}{*}{{\scalebox{1.75}\speechmod{}\scalebox{1.75}\videomod{}}} & \hyperlink{gemma3n}{Gemma 3n} & 35.1 & 73.0 & 26.2 & \multirow{5}{*}{\texttimes} & 58.9 & 71.5 & 25.1 & \multirow{5}{*}{\texttimes} \\
%  &  & \hyperlink{ming}{Ming-Lite-Omni} & 117.5 & 53.0 & 15.8 & & 128.2 & 53.3 & 13.3 & \\
%  &  & \hyperlink{minicpm}{MiniCPM-o-2} & 144.8 & 39.7 & 21.4 & & 207.1 & 38.8 & 23.1 & \\
%  &  & \hyperlink{ola}{Ola} & 104.1 & 76.6 & 37.3 &  & 98.8 & 76.3 & 37.0 &  \\
%  &  & \hyperlink{qwen2.5omni}{Qwen2.5-Omni} & 43.5 & 77.3 & 34.3 &  & 48.0 & 76.5 & 35.1 & \\
% \midrule
% \midrule
% \multirow{19}{*}{\rotatebox[origin=c]{90}{\scalebox{1.5}\longin{}}} & \multirow{7}{*}{{\scalebox{2}\textmod{}}} & \hyperlink{aya}{Aya Expanse} & \multirow{7}{*}{\texttimes}  & 68.7 & 26.7 & 17.0 & \multirow{7}{*}{\texttimes} & 68.7 & 23.1 & 16.3 \\
%  &  & \hyperlink{gemma3}{Gemma 3} &  & 85.5 & 22.9 & 5.6 &  & 83.4 & 21.8 & 5.2 \\
%  &  & \hyperlink{gptoss}{GPT-oss} &  & 75.0 & 24.6 & 10.5 &  & 70.1 & 20.9 & 9.2 \\
% &  & \hyperlink{llama3}{Llama 3.1} &  & 81.4 & 30.3 & \textbf{\underline{18.1}} &  & 79.5 & 31.0 & \textbf{\underline{17.3}} \\
%  &  & \hyperlink{phi4}{Phi4} &  & 84.5 & 30.8 & 7.3 &  & \textbf{\underline{84.7}} & 29.6 & 8.4 \\
%  &  & \hyperlink{qwen3}{Qwen3} &  & 84.8 & \textbf{37.9} & 14.1 &  & 84.5 & 35.6 & 14.0 \\
%  &  & \hyperlink{tower}{Tower+} &  & \textbf{\underline{85.6}} & 29.5 & 13.4 &  & 83.7 & 23.4 & 11.2 \\
%  \cmidrule{2-11}
%  & \multirow{5}{*}{{\scalebox{2}\speechmod{}}} & \hyperlink{desta2}{DeSTA2} & 112.9 & 41.3 & 12.5 & 0.8 & 132.5 & 40.8 & 12.6 & 1.3 \\
%  &  & \hyperlink{granite}{GraniteSpeech} & 99.9 & 36.0 & -23.7 & 0.4 & 80.4 & 34.6 & -22.8 & -12.0 \\
%  &  & \hyperlink{phi4m}{Phi4-Multimodal} & 39.2 & 59.7 & 37.6 & 4.5 & 29.8 & 59.5 & \textbf{37.3} & 13.2 \\
%   &  & \hyperlink{qwen2a}{Qwen2-Audio} & 92.9 & 41.0 & 28.8 & 4.6 & 93.1 & 41.1 & 28.9 & 4.6 \\
%  &  & \hyperlink{ultravox}{UltraVox v0.5} & 89.1 & 38.0 & 12.7 & -3.8 & 92.5 & 38.0 & 12.5 & -3.9 \\
%  \cmidrule{2-11}
%  & \multirow{5}{*}{{\scalebox{2}\videomod{}}} & \hyperlink{internvl3}{InternVL3} & \multicolumn{2}{c}{\multirow{5}{*}{\texttimes}} & 27.6 & 15.4 & \multicolumn{2}{c}{\multirow{5}{*}{\texttimes}} & 27.9 & 14.8 \\
% &  & \hyperlink{llavanv}{LLaVA-NeXT} & \multicolumn{2}{c}{} & 7.2 & -7.9 & & & 5.2 & -7.4 \\
%  &  & \hyperlink{qwen2.5vl}{Qwen2.5-VL} & \multicolumn{2}{c}{} & 33.7 & 17.3 & & & 34.9 & 14.6 \\
%  &  & \hyperlink{videollama3}{VideoLLaMA3} & \multicolumn{2}{c}{} & 26.8 & -18.5 & & & 26.5 & -34.6 \\
%  &  & \hyperlink{videoxl2}{Video-XL2} & \multicolumn{2}{c}{} & 17.2 & 2.1 & & & 17.4 & 2.8 \\
%  \cmidrule{2-11}
%  & \multirow{3}{*}{{\scalebox{1.75}\speechmod{}\scalebox{1.75}\videomod{}}} & \hyperlink{minicpm}{MiniCPM-o-2} & 98.7 & 51.1 & 21.5 & -3.2 & 98.2 & 39.1 & 22.9 & -4.0 \\
%  &  & \hyperlink{ola}{Ola} & \textbf{14.0} & 63.2 & 36.2 & 8.8 & \textbf{\underline{6.6}} & 58.7 & 36.2 & 9.9 \\
%  &  & \hyperlink{qwen2.5omni}{Qwen2.5-Omni} & 98.5 & 47.5 & 32.5 & 6.1 & 94.9 & 40.2 & 34.8 & 6.0 \\
%  \bottomrule
% \end{tabular}}
% \caption{Overall results, averaged across languages, on \MCIFFIX{} and \MCIFMIX{}, divided into the 4 macro-areas: recognition (\textbf{REC}), translation (\textbf{TRANS}), question answering (\textbf{QA}), and summarization (\textbf{SUM}). Best result by context is marked in \textbf{bold}, and best overall result is \underline{underlined}. \texttimes{} marks tasks that cannot be performed for a given modality and context: recognition is unavailable for LLMs and VideoLLMs, as it requires access to speech; translation cannot be done with VideoLLMs, since they lack both speech and transcripts; and summarization is not defined for short-form. Gemma 3n and Ming-Lite-Omni are removed from \longin{} as they are not able to process long-form inputs.}
% \label{tab:overall}
% \end{table}


%=================


% \begin{table*}[t]
%     \centering
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{l|c|cccc|ccc|c|ccc|cccc}
%     \toprule
%      &  & \multicolumn{7}{c|}{\textbf{TEXT} \textmod{}} & \multicolumn{8}{c}{\textbf{SPEECH} \speechmod{}} \\
%      \textbf{Model} & \textbf{Context} & \multicolumn{4}{c|}{\textbf{TQA}} & \multicolumn{3}{c|}{\textbf{MT}} & \textbf{ASR} & \multicolumn{3}{c|}{\textbf{ST} } &  \multicolumn{4}{c}{\textbf{SQA}}  \\
%     & &  en-en & en-de & en-it & en-zh & en-de & en-it & en-zh & en-en & en-de & en-it & en-zh & en-en & en-de & en-it & en-zh \\
%     \midrule
%     Qwen2.5-Omni & \multirow{2}{*}{\shortin{}} &  \multicolumn{4}{c|}{\multirow{2}{*}{\texttimes}}  & xx & xx & xx & xx \\ 
%     Phi4-Multimodal & & & & & & xx & xx & xx & xx & xx \\ 
%     \midrule
%     Qwen2.5-Omni & \multirow{2}{*}{\longin{}} & xx & xx & xx & xx & xx \\ 
%     Phi4-Multimodal &  & xx & xx & xx & xx & xx \\ 
%     \bottomrule
%     \end{tabular}%
%     }
%     \caption{Results for text and speech-text models using the metrics reported in \cref{subsec:metrics}.}
%     \label{tab:main_fix}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     \setlength{\tabcolsep}{4pt} 
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{c|l|c|ccc|cccc|cc|cccc}
%     \toprule
%      \multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Mod.}}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Con.}}}  & \multicolumn{3}{c|}{\textbf{TEXT} \textmod{}} & \multicolumn{4}{c|}{\textbf{SPEECH} \speechmod{}} & \multicolumn{2}{c|}{\textbf{VIDEO} \videomod{}} & \multicolumn{4}{c}{\textbf{AUDIO-VIDEO} \speechmod{}\videomod{}} \\
%      & &  & \textbf{TQA}$\uparrow$ & \textbf{TSUM}$\uparrow$ & \textbf{MT}$\uparrow$ & \textbf{ASR}$\downarrow$ &  \textbf{SQA}$\uparrow$ & \textbf{SSUM}$\uparrow$ & \textbf{ST}$\uparrow$ & \textbf{VQA}$\uparrow$ & \textbf{VSUM}$\uparrow$ & \textbf{AVR}$\downarrow$ & \textbf{AVQA}$\uparrow$ &  \textbf{AVSUM}$\uparrow$ & \textbf{AVT}$\uparrow$  \\
%     \midrule
%     \multirow{5}{*}{\rotatebox[origin=c]{90}{\speechmod{}}} & DeSTA2 & \multirow{10}{*}{\rotatebox[origin=c]{90}{\shortin{}}} &  \multicolumn{3}{c|}{\multirow{10}{*}{\texttimes}}  & 45.1 & xx & \multirow{2}{*}{\texttimes} & 75.5 & xx & \multirow{5}{*}{\texttimes} & x & x & \multirow{5}{*}{\texttimes} & x \\ 
%     & GraniteSpeech & & & & & xx & xx & & xx & xx & & \\
%     & Phi4-Multimodal & & & & & 6.8 & xx & & 80.2 & xx & & \\
%     & Qwen2-Audio & & & & & 31.3 & xx & & 74.7 & xx & & \\
%     & UltraVox & & & & & 146.2 & xx & & 44.3 & xx & & \\ 
%     \cmidrule{1-2} \cmidrule{7-16}
%     \multirow{5}{*}{\rotatebox[origin=c]{90}{\videomod{}}} & InternVL3 & & & & & 45.1 & xx & \multirow{2}{*}{\texttimes} & 75.5 & xx & \multirow{5}{*}{\texttimes} & x & x & \multirow{5}{*}{\texttimes} & x \\ 
%     & Qwen2.5-VL & & & & & xx & xx & & xx & xx & & \\
%     & VideoLLaMA3 & & & & & 6.8 & xx & & 80.2 & xx & & \\
%     & Video-XL2 & & & & & 31.3 & xx & & 74.7 & xx & & \\
%     & LLaVA-NeXT & & & & & 146.2 & xx & & 44.3 & xx & & \\ 
%     \midrule
%     \midrule
%     & Qwen2.5-Omni & \multirow{2}{*}{\rotatebox[origin=c]{90}{\longin{}}} & xx & xx & xx & xx & xx \\ 
%     & Phi4-Multimodal &  & xx & xx & xx & xx & xx \\ 
%     \bottomrule
%     \end{tabular}%
%     }
%     \caption{Results on \MCIFMIX{} of the XX models for each supported input modality (\textbf{Mod.}) and context (\textbf{Con.}) using the metrics reported in \cref{subsec:metrics}.}
%     \label{tab:main_fix}
% \end{table*}






% Breakdown on the 4 tasks macro-area:

% RECOGNITION: SpeechLLMs are in general better in recognition in the short form but Ola, an MLLM, is the best in the long form by a large margin, except for Phi4 Multimodal, which still scores about 20+ WER. Overall, performance degrades a lot when switching to long-form.

% TRANSLATION: As expected, I would say, LLMs are in general better in translation. Some short-form SpeechLLMs and MLLMs are competitive but the results are consistently worse in the long-form scenario. This is particularly evident in SpeechLLMs, in which we have a drop of up to 30 COMET points for some languages.

% QUESTION-ANSWERING: Results on QA are more mixed, especially in the short form, in which all SpeechLLMs, VideoLLMs, and MLLMs scored at least one best result. Still in the short form, we have competitive (at least, with scores >30) models in both SpeechLLMs (Phi4multi and Qwen2Audio) and MLLMs (Ola, Qwen2.5Omni) while only Qwen2.5-VL shows to be especially competitive in Chinese. In the long form, both Ola and Qwen2.5Omni are very competitive, with Qwen2.5Omni scoring the best results in both English and Chinese, I guess it is connected to the language distribution in the training set. The degradation seen in the other two tasks, recognition and translation, seems to affect less QA if we consider MLLMs, which instead see their results almost always improved or on par when switching to long-form. Instead, coherently with recognition and translation, SpeechLLMs and VideoLLMs see an important performance drop when passing from short to long-form context. An interesting aspect is that, in general, LLMs are not good in this task, while I was thinking about the opposite.

% SUMMARIZATION: to be included.

% SHORT vs LONG considerations: short better results than long, but with some exceptions as Ola (analyzed in \cref{subsec:modalities}). Upon manual inspection, we found that Ola misinterprets the prompt to transcribe and does image captioning with the slides instead in the short-form audio. Instead, common phenomena of this decrease in performance is due to Undertranslation (desta/qwen/phi), that is only part of the context is translated. This is likely what happens with tower.
% Instead, there are some models that, independently from the short or long context either use the wrong language (English): graniteSpeech or refuse to answer: ultra vox. 

% Ola cuts and concatenate the embeddings of speech, 30s each, as they leverage Whisper encoder, probably, that is why it is good on long audio. The long-form component is not handled on the encoder part but it is in charge of the LLM to support such long concatenated embeddings.



\REClabelfull{} Some SpeechLLMs (Phi4-Multimodal and GraniteSpeech) and MLLM (Gemini 2.5 Flash) show strong performance (WER$<$10), demonstrating the feasibility of this macro-task. However, despite being the simplest one--and on which all models are trained on--several systems fail in one or both context types. UltraVox v0.5\speechmodsmall{}, Ming-Lite-Omni\speechmodsmall{}\videomodsmall{}, and MiniCPM-o-2\speechmodsmall{}\videomodsmall{} achieve scores superior to 100 WER on both short- and long-form, DeSTA2\speechmodsmall{} exceeds 100 WER on long-form, and, surprisingly, Ola\speechmodsmall{}\videomodsmall{} drops sharply from 6.6/14.0 (long-form) to 98.8/104.1 (short-form). A manual inspection of the model's outputs revealed that Ola often misinterprets transcription prompts in short-form, opting instead to perform image captioning of accompanying slides, while this is not the case for long-form inputs (see Example 1 in \cref{app:examples}). The long-form results of Ola also suggest that its architecture--particularly the strategy of chunking and concatenating long speech segments using a Whisper-based encoder--enables the model to obtain high transcription quality over extended inputs. 


% Most SpeechLLMs show good performance on short-form audio, confirming their specialization in ASR, while, among MLLMs, only Gemini 2.5 Flash obtains good results. However, SpeechLLMs' performance degrades significantly in the long-form scenario.
% In contrast, the MLLMs Ola and Gemini 2.5 Flash achieve the best long-form performance... 
% Ola\speechmodsmall{}\videomodsmall{}, achieves the best long-form performance, followed by Gemini 2.5 Flash\speechmodsmall{}\videomodsmall{}, and outperforming SpeechLLMs, including Phi4-Multimodal\speechmodsmall{}, which reports a WER above 30. This suggests that Ola's architecture--particularly its strategy of chunking and concatenating long speech segments using a Whisper-based encoder--enables it to maintain transcription quality over extended inputs. Despite this, long-form recognition remains a major challenge for most models.
% fattibili, speechllm che mllm, nonostante sia un task semplice, alcuni modelli non sono capaci di fare il task con WER sopra 100, alcuni in tutte le ocndizioni e altri no (long e short)

\TRANSlabelfull{} 
% As expected, LLMs dominate in this task, benefiting from the fact that processing text is an easier--as it starts from human transcripts--and more advanced task, a trend that is also consistent across target languages (see \cref{app:mcif_extended}). Beyond LLMs, some SpeechLLMs and MLLMs achieve competitive results with COMET scores above 75 with DeSTA2\speechmodsmall{}, Ola\speechmodsmall{}\videomodsmall{} and Qwen2.5-Omni\speechmodsmall{}\videomodsmall{}, and even exceeding 80 in the case of Phi4-Multimodal\speechmodsmall{}. Similarly to recognition, some models are not able to perform the task in all conditions (UltraVox v0.5\speechmodsmall{}, and MiniCPM-o-2\speechmodsmall{}\videomodsmall{}), or in long-form (DeSTA2\speechmodsmall{}, GraniteSpeech\speechmodsmall{}, Qwen2-Audio\speechmodsmall{}, and Qwen2.5-Omni\speechmodsmall{}\videomodsmall{}) showing COMET $<$ 50. The degradation is frequently attributable to under-translation, where models fail to translate the entire context, a phenomenon that is more pronounced with long-form inputs. An exception is Gemini 2.5 Flash\speechmodsmall{}\videomodsmall{}, which performs better on long-form inputs; manual inspection shows that with shorter segments it hallucinates or over-elaborates on video or audio content--a known issue in current LLMs \citep{briakou2024implications}.
As expected, LLMs dominate due to the maturity of text-based translation, a trend consistent across target languages (see \cref{app:mcif_extended}). Beyond LLMs, some SpeechLLMs and MLLMs achieve competitive results in short-form, with COMET $>$75 for DeSTA2\speechmodsmall{}, Ola\speechmodsmall{}\videomodsmall{}, and Qwen2.5-Omni\speechmodsmall{}\videomodsmall{}, and even $>$80 for Phi4-Multimodal\speechmodsmall{}. However, several models fail to perform this task, either across all conditions (UltraVox v0.5\speechmodsmall{}, MiniCPM-o-2\speechmodsmall{}\videomodsmall{}) or on long-form (DeSTA2\speechmodsmall{}, GraniteSpeech\speechmodsmall{}, Qwen2-Audio\speechmodsmall{}, Qwen2.5-Omni\speechmodsmall{}\videomodsmall{}), where scores drop below 50 COMET. The degradation is often due to under-translation, with models skipping parts of the context--especially in long-form (see Example 2 in \cref{app:examples}). An exception is Gemini 2.5 Flash\speechmodsmall{}\videomodsmall{}, which performs better on long-form; a manual inspection revealed that, on shorter segments, it hallucinates or over-elaborates on audio/video content (see Example 3 in \cref{app:examples}), a known issue in current LLMs \citep{briakou2024implications}.

\QAlabelfull{} 
% It shows inconsistent results, especially in short-form, where best-performing models for each language span SpeechLLMs (Phi4Multimodal), VideoLLMs (Qwen2.5-VL), and MLLMs (Gemini 2.5 Flash). However, Gemini 2.5 Flash\speechmodsmall{}\videomodsmall{} stands out in long-form, constantly achieving the best results, with an average BERTScore above 45 on all target languages (see \cref{app:mcif_extended}). Instead, SpeechLLMs and VideoLLMs experience significant drops, mirroring trends seen in the other tasks. Only few models are incapable of performing the task, with very low performance (BERTScore $<$ 10) in the case of LLaVA-NeXT\videomodsmall{} or approaching 0 or even being negative in the case of GraniteSpeech\speechmodsmall{}, indicating random outputs in the same or different languages, respectively. 
Surprisingly, not all LLMs excel in question answering even if provided with human transcripts, as the best performance consistently comes from Gemini 2.5 Flash\speechmodsmall{}\videomodsmall{}.
Results are inconsistent, particularly in short-form, where the top models vary by language (see \cref{app:mcif_extended}): SpeechLLMs (Phi4-Multimodal), VideoLLMs (Qwen2.5-VL), and MLLMs (Gemini 2.5 Flash). In contrast, Gemini 2.5 Flash\speechmodsmall{}\videomodsmall{} clearly dominates in long-form, consistently ranking first across languages with average BERTScores above 45. SpeechLLMs and VideoLLMs, instead, suffer significant performance drops, echoing trends observed in other tasks. Only a few models fail entirely, such as LLaVA-NeXT\videomodsmall{} (BERTScore $<$10, corresponding to outputs in the wrong language; see Example 4 in \cref{app:examples}) and GraniteSpeech\speechmodsmall{} (BERTScore around 0, corresponding to random text in the correct language or the transcript of the content; see Example 5 in \cref{app:examples}). 
% , underscoring the limitations of pure LLMs in crosslingual information extraction over extended contexts.
%These tasks show mixed results, especially in short-form, where top models span SpeechLLMs, VideoLLMs, and MLLMs. SpeechLLMs like Phi4-Multimodal and Qwen2-Audio, and MLLMs like Ola and Qwen2.5-Omni, achieve BERTScores above 30 across languages, while Qwen2.5-VL leads among VideoLLMs, notably in Chinese (see \cref{app:mcif_extended}). Unlike recognition and translation, MLLMs maintain or improve performance on long-form QA, with Ola and Qwen2.5-Omni remaining competitive, whereas SpeechLLMs and VideoLLMs drop significantly. Surprisingly, the best QA scores often come from Qwen2.5-VL, and in long-form, Phi4-Multimodal tops \MCIFMIX{}, highlighting LLM limitations in crosslingual extraction over extended contexts.

\SUMlabelfull{} 
% It is by far the most challenging, with some systems even yielding negative BERTScore scores--meaning that they are worse than a system producing random outputs in the target language--among SpeechLLMs (GraniteSpeech, Ultravox), VideoLLMs (LLaVA-NeXT, VideoLLaMA3), and MLLMs (MiniCPM-o-2). Manual inspection reveals two main sources of failure: models either default to the wrong language (often English for all tasks) or disregard the instruction entirely (e.g., LLaVA-NeXT\videomodsmall{} transcribes slides instead of summarizing them). In contrast, LLMs perform best at summarization, facilitated by human transcripts, and are followed by VideoLLMs, whose results fluctuate widely between complete failure and strong performance (InternVL3, Qwen2.5-VL). MLLMs show a similar instability, though at generally lower BERTScore. SpeechLLMs struggle the most, with the sole exception of Phi4-Multimodal\speechmodsmall{}.
This is by far the most challenging macro-task, with some systems even producing negative BERTScores--worse than random outputs in the target language. Failures span SpeechLLMs (GraniteSpeech, UltraVox v0.5), VideoLLMs (LLaVA-NeXT, VideoLLaMA3), and MLLMs (MiniCPM-o-2). Manual inspection points to two recurring issues: models either default to the wrong language (often English across tasks; see Example 4 in \cref{app:examples}) or ignore the instruction altogether (e.g., LLaVA-NeXT\videomodsmall{} transcribes slides instead of summarizing them; see Example 1 in \cref{app:examples}).
LLMs achieve the strongest results, confirming that text-only inputs remain easier to handle, followed by VideoLLMs, whose performance fluctuates widely between complete failure (LLaVA-NeXT and VideoLLaMA3) and strong outcomes (InternVL3 and Qwen2.5-VL). MLLMs exhibit similar instability, although generally at lower BERTScores. SpeechLLMs remain weak, with the sole exception of Phi4-Multimodal\speechmodsmall{}.

% on \MCIFMIX{}, highlighting a pronounced sensitivity to prompt variation.

% PROBLEM WITH VISION SUMMARIES (by Bea):  
% - LLava. Out of 20 summaries that I checked, only 7 seem well-formed and related to the instruction. The rest is very hallucinated  (e.g. sample id 2 = "The image shows a cityscape with a river running through it. The cityscape is surrounded by buildings on both sides. The river is lined with trees and has a bridge in the middle. The sky is clear and blue". The model always makes the same error, which is it tries to describe an invented image.
% - Models tend to summarize using the third person (e.g. the authors state that...) whereas our abstracts are in the first person (I/we state...). Just something to keep in mind that could be penalized in the eval

\scalebox{1.25}\shortin{} \scalebox{1.25}\battle{} \scalebox{1.25}\longin{} 
%%%%% OLD
% Across tasks, short-form performance is generally stronger, with long-form leading to clear degradation in most models, particularly SpeechLLMs and VideoLLMs. An exception is Gemini 2.5 Flash\speechmodsmall{}\videomodsmall{}--with significant improvements in all tasks--and Ola\speechmodsmall{}\videomodsmall{} in the recognition task--showing a significant improvement from short- to long-form context inputs of more than 45 WER.  Despite this, long-form recognition remains a major challenge for most models.
% % A manual inspection of the model's outputs revealed that Ola often misinterprets transcription prompts in the short-form, opting instead to perform image captioning of accompanying slides, while this is not the case for long-form inputs. 
% For other models, the primary cause of long-form degradation appears to be undergeneration, where only part of the context is generated. Additional failure cases include persistent use of the wrong language (e.g., GraniteSpeech\speechmodsmall{} defaulting to English) or refusal to answer the user's requests (UltraVox v0.5\speechmodsmall{}), independent of context type.
% %%%%FROM RECOGNITION
% Most SpeechLLMs show good performance on short-form audio, confirming their specialization in ASR, while, among MLLMs, only Gemini 2.5 Flash obtains good results. However, SpeechLLMs' performance degrades significantly in the long-form scenario.
% In contrast, the MLLMs Ola and Gemini 2.5 Flash achieve the best long-form performance... 
% Ola\speechmodsmall{}\videomodsmall{}, achieves the best long-form performance, followed by Gemini 2.5 Flash\speechmodsmall{}\videomodsmall{}, and outperforming SpeechLLMs, including Phi4-Multimodal\speechmodsmall{}, which reports a WER above 30. Despite this, long-form recognition remains a major challenge for most models.
% %%%%%%FROM TRANSLATION
% While some SpeechLLMs and MLLMs are competitive on short-form, performance deteriorates markedly in the long-form setting, by up to 34 COMET points for SpeechLLMs.
% %%%%%% FROM QA
% In contrast to recognition and translation, most MLLMs generally improve or maintain performance on long-form question answering, particularly Ola\speechmodsmall{}\videomodsmall{} and Qwen2.5-Omni\speechmodsmall{}\videomodsmall{}.
%%%% NEW
Across tasks, models generally perform better on short-form inputs, with long-form leading to notable degradation--particularly for SpeechLLMs and VideoLLMs. An exception is Gemini 2.5 Flash\speechmodsmall{}\videomodsmall{}--with significant improvements in all tasks--and Ola\speechmodsmall{}\videomodsmall{} in recognition. Despite this, long-form recognition remains a major challenge for most systems, regardless of their input modality. Manual inspection revealed that the main source of degradation is under-generation, with models producing only partial outputs (see Example 2 in \cref{app:examples}). This is particularly common in recognition but also in translation: for instance, DeSTA2\speechmodsmall{} and Qwen2-Audio\speechmodsmall{} drop by about 34 COMET, while Qwen2.5-Omni\speechmodsmall{}\videomodsmall{} falls by roughly 30 COMET. In contrast, most MLLMs improve or maintain performance on long-form question answering, notably Ola\speechmodsmall{}\videomodsmall{} and Qwen2.5-Omni\speechmodsmall{}\videomodsmall{}. Additional failure cases that are especially pronounced in long-form settings include persistent use of the wrong language (GraniteSpeech\speechmodsmall{} defaulting to English; see Example 4 in \cref{app:examples}), common in all macro-tasks, or refusal to answer the user's requests (UltraVox v0.5\speechmodsmall{}; see Example 6 in \cref{app:examples}). Lastly, some MLLMs (Gemma 3n and Ming-Lite-Omni) cannot handle long-form inputs at all, constrained by limited context windows.
% Overall, long-form inputs expose weaknesses in multimodal integration, context coverage, and language adherence, highlighting critical areas for future MLLM development.

\textbf{\MCIFFIX{} \scalebox{1.25}\battle{} \MCIFMIX{}.} 
Comparing the two \DATASETNAME{} variants reveals that most models exhibit limited robustness to prompt reformulation, with sensitivity varying across tasks. Recognition is the most affected: some SpeechLLMs (DeSTA2, and UltraVox v0.5) and MLLM (MiniCPM-o-2) fluctuate by more than 60 WER on short-form, and nearly all systems vary on long-form, with shifts up to 20 WER (e.g., GraniteSpeech\speechmodsmall{}). Translation remains relatively stable for LLMs, even if drops of up to 4.9 COMET occur (e.g., GPT-oss), with SpeechLLMs showing similar patterns. MLLMs prove less reliable, particularly in long-form, with MiniCPM-o-2\speechmodsmall{}\videomodsmall{} losing up to 12 COMET. Question answering is generally stable, but most LLMs show notable variations, with changes up to 6.1 BERTScore (Tower+). Summarization follows an unclear trend, as some models show little robustness to prompt reformulation (GraniteSpeech\speechmodsmall{}, Phi4-Multimodal\speechmodsmall{}, VideoLLaMA3\videomodsmall{}), with variations up to 16.1 BERTScore, while others remain consistent.
% Overall, only a few systems demonstrate strong robustness to prompt reformulation across tasks, and mostly on short-form.

%%%%% EXTENDED VERSION 2
% When comparing results obtained on \MCIFFIX{} and \MCIFMIX{}, we observe notable variations in performance trends, revealing which models are more robust to prompt variation. In the recognition task, performance drops are particularly severe: DeSTA2 and UltraVox degrade by up to 46.6 WER on \shortin{}, with DeSTA2 also losing nearly 40 WER on \longin{}. Among MLLMs, MiniCPM-o-2 sees its WER nearly double on \shortin{}, while Qwen2.5-Omni and Ming-Lite-Omni also drop by 5.11 WER. Even Ola, the strongest model on long-form recognition, suffers a $\sim$27 WER drop under prompt variation. In translation, while LLMs are generally more robust, they show some degradation (up to 4 COMET). SpeechLLMs follow a similar trend, aside from UltraVox, which shows both degradation (-9.2 COMET on Italian) and improvement (+10.6 on Chinese). Comparable but smaller inconsistencies are also observed with Phi4-Multimodal on \longin{}. Question answering is similarly affected. We observe drops of up to 6 BERTScore, especially in Chinese for Phi4-Multimodal and up to 4.6 for LLaVA-NeXT. MLLMs are also impacted, with Ming-Lite-Omni and Qwen2.5-Omni degrading by 5.5 and 6.9 BERTScore, respectively, but also exhibiting isolated gains (e.g., MiniCPM-o-2 +29.3 on English \longin{}). For the summarization task, \waiting{}.
% In terms of best-performing models, Phi4-Multimodal continues to lead in \shortin{} recognition and translation, achieving the best recognition score and showing strong robustness to prompt changes. Question answering results remain mixed, with shifts in model rankings compared to \MCIFMIX{}. On \longin{} recognition, Phi4-Multimodal also achieves the top score, as Ola--the best model on \MCIFFIX{}--suffers a significant performance drop. In translation, LLMs retain their advantage, but with relative rankings shift: Phi4 and Tower+ outperform Gemma on Italian and Chinese, while Qwen3 surpasses Tower+ on German. For question answering, Qwen2.5-Omni demonstrates strong robustness to prompt variation, especially on \longin{}, securing two of the four best overall scores. These results reveal that many current models lack robustness to prompt reformulation of \MCIFMIX{}, with some tasks amplifying this vulnerability (e.g., recognition). 

%%%% EXTENDED VERSION
% When comparing results obtained on \MCIFFIX{} and \MCIFMIX{}, we observe notable variations in performance trends, revealing which models are more robust to prompt variation. In the recognition task, several models exhibit substantial degradation, but not universally. Among SpeechLLMs, DeSTA2 and UltraVox show significant WER increases of 27.8 and 46.6, respectively, on \shortin{}. This trend extends to \longin{}, particularly for DeSTA2, which experiences a 39.7-point degradation. Among MLLMs on \shortin{}, MiniCPM-o-2 is heavily impacted, with WER nearly doubling, while Qwen2.5-Omni and Ming-Lite-Omni also show declines of 5-11 WER. On \longin{}, degradation is observed only for Ola ($\sim$27 WER), while Qwen2.5-Omni and MiniCPM-o-2 maintain performance similar to \MCIFFIX{}. In the translation task, LLMs remain largely stable under prompt variation, with rare performance drops. A similar pattern holds for SpeechLLMs across both \shortin{} and \longin{}, except for UltraVox on \shortin{}, which shows a 9.2-point drop on Italian but an unexpected 10.6-point gain on Chinese. A comparable inconsistency, though less pronounced, is seen with Phi4-Multimodal on \longin{}. In question answering, we observe degradations of up to 6 BERTScore, particularly in Chinese with Phi4-Multimodal. VideoLLMs follow similar trends, with LLaVA-NeXT experiencing a 4.6-point drop in Chinese, but Video-XL2 showing gains of up to 4.2 in German. MLLMs are also sensitive to prompt variation, with performance drops of up to 5.5 BERTScore for Ming-Lite-Omni on \shortin{} and 6.9 for Qwen2.5-Omni on \longin{}. However, we also observe notable improvements--Ming-Lite-Omni gains 18.5 BERTScore on German \shortin{}, and MiniCPM-o-2 gains 29.3 on English \longin{}. For the summarization task, \waiting{}. In terms of best-performing models, Phi4-Multimodal continues to lead in \shortin{} recognition and translation, achieving the best transcription score and showing strong robustness to prompt changes. Question answering results remain mixed, with shifts in model rankings compared to \MCIFMIX{}. On long-form recognition, Phi4-Multimodal again achieves the top score, as Ola suffers a significant performance drop. In translation, LLMs retain their advantage, but relative rankings shift: Phi4 and Tower+ outperform Gemma on Italian and Chinese, while Qwen3 surpasses Tower+ on German. For question answering, Qwen2.5-Omni demonstrates strong robustness to prompt variation, especially on \longin{}, securing two of the four best results overall.

% To sum up, results on both \MCIFFIX{} and \MCIFMIX{} highlight that summarization is the most difficult task for all models, and integrating another modality than text (either speech and/or video) does not lead to improved performance in current models. Conversely, QA benefits from the addition of both speech and video modality. LLMs still lead the translation task, while recognition is the most affected task in the presence of prompt variability of \MCIFMIX{}. Lastly, long-form processing is another prevalent challenge in most models, which see their performance dropping compared to short-form for all tasks and languages.


To sum up, results reveal consistent trends in current models' performance. Summarization is the most difficult task, with no gains from adding speech or video to text--underscoring limitations in multimodal integration. QA shows the opposite pattern, benefiting from speech or video and highlighting the value of non-textual modalities. LLMs continue to lead in translation, while recognition proves highly sensitive to prompt variability. Long-form proves to be challenging, with nearly all models suffering significant drops across tasks compared to short-form, especially SpeechLLMs and MLLMs. Together, these findings expose the wide gap between current systems and the goal of robust, multimodal, crosslingual instruction following, pointing to clear avenues for future progress.


%%%%%%%% IN PENDING
% \textbf{Open \scalebox{1.25}\battle{} Closed Models.}  \waiting{} % All models compared to Gemini

% These findings highlight the growing but uneven capabilities of current multimodal systems, especially when tasked with long-form, crosslingual, and instruction-driven inputs. MCIF provides a comprehensive framework to expose these limitations and guide future advancements.


\subsection{Effect of Modalities Integration}
\label{subsec:modalities}

Since \DATASETNAME{} is completely parallel across languages and modalities, 
% it allows for investigating the effectiveness of integrating different modalities into LLMs. 
it enables an ablation study on how different modalities contribute to MLLM performance. Specifically, we evaluate each model under four input conditions: text only, speech only, video only, and speech+video (as already reported in \cref{tab:overall}).
% For this study, we task each MLLM to use either text only, the speech modality, the video modality, or both the speech and video modalities (as already reported in \cref{tab:overall}). 
To isolate the contribution of each modality, we use the \MCIFFIX{} set to avoid biases from the single fixed prompt in \MCIFFIX{} that could favor some models over others, and run the evaluation on both short and long contexts. The results are shown in \cref{fig:modality-bar}.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\linewidth]{barplot.pdf}
    \caption{
    % MLLMs results over \MCIFMIX{} depending on the modality leveraged during inference. Results are averaged across languages.
    MLLM results on \MCIFMIX{} by inference modality, averaged across languages.}
    \label{fig:modality-bar}
\end{figure}

% In recognition, we observe that, as expected, the speech modality is essential to drive the task but we also notice that the video modality is not of help and, instead, the performance degrades significantly when both modalities are enabled in all but one case (i.e., Ola on long-form). In translation, the leading modality is again speech on short-form, with the only exception of Ola, benefiting from the additional video modality (with gains of XX), and text on long-form--which is only present with this context--and followed by the speech modality. In short-form question answering, the speech modality is again fundamental, with the video modality lagging behind in all but one case, where anyway the gains are minimal (X vs Y). Instead, in long-form question answering, we observe a negative score from MiniCPM-o-2 when only the video modality is used, which, in accordang with the short-form trends, is the least useful modality. With the long-form context, we also observe that the joint processing of speech and video modalities are of help in two cases out of three (MiniCPM-o-2 and Qwen2.5-Omni). In summarization, trends are less clear, but in two out of three cases, the textual modality is the one enabling the best or comparable performance. Even in this task, we observe negative scores with the video-only modality (MiniCPM-o-2 and Ola) but also when both the speech and video modalities are enabled (MiniCPM-o-2). Overall, the results suggest that MLLMs still struggle to successfully integrate both speech and video modalities together, often producing the opposite effect instead of being helpful. It also emerges that the vision modality, which proved to be particularly useful in question answering (\cref{tab:overall}), is not exploited properly by current MLLMs, always yielding the lowest results. Moreover, the superior performance obtained by the text-only modality on long-form translation indicates a room for improvement on the effectively integration of the speech modality into LLMs, especially under a crosslingual point of view. 

In recognition, comparing Speech and Speech+Video both in short- and long-form, we observe that the video modality provides no benefit and often degrades performance when combined with speech--except in one case (Ola on long-form). In translation, speech leads the performance in short-form, with Ola being the only model gaining from the addition of video (improving by 8.6 COMET), while in long-form the text modality--available only in this setting--dominates,  followed by speech. For short-form question answering, speech again proves fundamental, while video consistently underperforms. 
% Even in the single case where video performs better, i.e., Qwen2.5-Omni, the margin over speech-only is small (1.9 BERTScore), and this is also the only model where combining speech and video yields a clear benefit over speech alone.
The only case where video outperforms speech is Qwen2.5-Omni, but the margin is minimal (1.9 BERTScore); notably, it is also the only model where combining speech and video brings a clear gain over speech alone.
In long-form question answering, video alone yields negative scores (MiniCPM-o-2), confirming its limited exploitation in current MLLMs, but joint speech-video processing shows benefits in two out of three models (MiniCPM-o-2 and Qwen2.5-Omni). Summarization trends are less consistent across systems: in two out of three models, text enables the best or comparable results, while video-only produces negative scores (MiniCPM-o-2 and Ola), and joint speech-video processing even harms performance in one case (MiniCPM-o-2). Overall, these findings indicate that current MLLMs struggle to effectively integrate speech and video, with the joint multimodal processing often not being of any help or even counterproductive. Moreover, the video modality--despite showing the best results in short-form question answering (\cref{tab:overall})--remains underutilized in MLLMs, systematically yielding the weakest results. 


% Finally, the superior performance of text-only inputs in long-form translation underscores the need for better integration of speech into LLMs, particularly in crosslingual settings.


% MLLMs with text, speech, video, and speech+video, analysis of the modalities: we see how MLLMs perform with different inputs, but the same prompt



\subsection{Breakdown on Question Answering}
\label{subsec:questions}

% To understand the performance of the models on various question types (\cref{subsec:annotations}), we break down the results by question modality (Audio-Visual, Audio, and Video) and source (General, Abstract, Transcript). 
To better understand model behavior beyond overall QA scores, we analyze performance across different question types (\cref{subsec:annotations}). Breaking results down by question modality (Audio-Visual, Audio, and Video) and by source (General, Abstract, Transcript) helps reveal how well models exploit specific input signals and how they handle varying levels of specificity and difficulty.
% To maximize the model types and prompt variability, we provide results on \MCIFMIX{} for the long context, as it covers all models, and average across languages. 
\begin{wrapfigure}[15]{r}{0.7\textwidth}
\includegraphics[width=0.7\textwidth]{radar.pdf}
\vspace{-15pt}
\caption{Performance breakdown on \MCIFMIX{} \longin{} QA of the best models by question modality and source.}\label{fig:qa-spider}
\end{wrapfigure} 
% In \cref{fig:qa-spider}, we show the results of the best model for each type (LLM, SpeechLLM, VideoLLM, and MLLM), namely: Qwen3, Phi4-Multimodal, Qwen2.5-VL, and Ola. Not Answerable (NA) scores are omitted since they are low (1 to 7 BERTScore) for all systems. 
% Upon manual inspection, we found that all models, regardless of input modality, attempt to answer Not Answerable questions even when the required information is unavailable. As a result, they often hallucinate responses, which are heavily penalized by BERTScore during evaluation.
% For this analysis, we report \MCIFMIX{} results on long contexts (averaged across languages) and show the best model for each family (Qwen3, Phi4-Multimodal, Qwen2.5-VL, Ola) in \cref{fig:qa-spider}. NA scores are omitted since they are consistently low for all models (in the 1-7 range), and a manual inspection revealed that they often hallucinate answers even when no information is available.
For this analysis, we use long-form contexts, which enable evaluation of all models, including LLMs, and report results on \MCIFMIX{} to avoid biases from the single fixed prompt in \MCIFFIX{}, which could favor some models over others. Scores are averaged across languages, and the best model from each family--Qwen3, Phi4-Multimodal, Qwen2.5-VL, and Ola--is shown in \cref{fig:qa-spider}.
% We observe that the A questions, relying on audio only, are better addressed by the SpeechLLM, and, coherently, the VideoLLM obtains the highest score on video only (V) questions. Surprisingly, the LLM--working on transcripts--achieves the better result (44 BLEUScore) on audiovisual questions (AV), followed by the SpeechLLM and the MLLM, who obtained the same score (42.6). As expected, the performance of the SpeechLLM on V questions and of the VideoLLM on A questions drop significantly (from 7 to 13 points), although they are still above 35, probably due to the help of the entire context. These scores highlight that, although specifically designed to process multiple modalities, MLLMs still struggle to leverage both speech and audio modalities when generating their outputs, suggesting a big room for improvement towards this direction. Looking at the question source, we notice instead similar performance trends among model types: common questions (General) obtained by far the highest scores (47.6-49.0), followed by more \textit{extractive} questions based either on transcripts, with scores oscillating between 33.7 and 36.6, or abstracts, with scores ranging from 23.2 to 27.0. In this case, the performance suggest that current models are significantly better at capturing and delivering generic information (e.g., the title of the paper or the affiliations) but still struggle with specific questions that should be exactly extracted from the input content, disregarding its modality.
% We observe that questions based on audio-only (A) are best handled by the SpeechLLM, and the VideoLLM better handle video-only (V) questions, while MLLMs are underperforming even if accessing both modalities. 
We find that audio-only (A) questions are best handled by the SpeechLLM, while the VideoLLM performs strongest on video-only (V) questions. Surprisingly, MLLMs underperform even if accessing both modalities.
The LLM, despite working only on transcripts, achieves the highest score on audiovisual (AV) questions (44), slightly surpassing both the SpeechLLM and MLLM (42.6), confirming that text remains easier to process than multimodal inputs. As expected, modality mismatches cause substantial drops: SpeechLLMs underperform on V questions and VideoLLMs on A questions (losses of 7-13 points), though both remain above 35, likely thanks to contextual cues. 
These results reveal that, despite being explicitly designed for multimodality, MLLMs still fail to effectively integrate speech and visual signals together, leaving substantial room for improvement.
Breaking results down by question source reveals a consistent trend: generic questions (General) yield the highest scores (47.6-49.0), while \textit{talk-specific} ones prove more challenging as performance drops to 33.7-36.6 on Transcript questions and further to 23.2-27.0 on Abstracts. This suggests that current models excel at retrieving common information (e.g., paper title or affiliations) but remain weak at retrieving fine-grained content, regardless of modality.


% \waiting{} Work in progress...

% performance breakdown based on the question types by modality (AV/V/A/NA) and source (generic, abstract, or content)  -- spider web instead of tables

% \section{Analyses}
% \label{sec:analyses}
